Fixpoint Approximation of Strategic Abilities under Imperfect Information

Model checking of strategic ability under imperfect information is known to be hard. The complexity results range from NP-completeness to undecidability, depending on the precise setup of the problem. No less importantly, fixpoint equivalences do not generally hold for imperfect information strategies, which seriously hampers incremental synthesis of winning strategies. In this paper, we propose translations of ATLir formulae that provide lower and upper bounds for their truth values, and are cheaper to verify than the original specifications. That is, if the expression is verified as true then the corresponding formula of ATLir should also hold in the given model. We begin by showing where the straightforward approach does not work. Then, we propose how it can be modified to obtain guaranteed lower bounds. To this end, we alter the next-step operator in such a way that traversing one's indistinguishability relation is seen as atomic activity. Most interestingly, the lower approximation is provided by a fixpoint expression that uses a nonstandard variant of the next-step ability operator. We show the correctness of the translations, establish their computational complexity, and validate the approach by experiments with a scalable scenario of Bridge play.

==> maintext.tex <==
\section{Underapproximating ATL\textsubscript{\lowercase{ir}}}\label{secUnder}

Following~\cite{Schobbens04}, we denote the satisfaction in the vanilla \ATL and \AMC
by $\satisf[\IR]$ and $\modelsmu$, respectively. \ATL can be embedded into
\AMC using the translation that assigns to a formula $\phi\in\ATL$ the formula
$\translIR(\phi)\in\AMC$ defined recursively as follows~\cite{AlurHK02}:
$\translIR(p) = p$, $\translIR(\neg\phi) = \neg\translIR(\phi)$,
$\translIR(\phi\lor\psi) = \translIR(\phi)\lor\translIR(\psi)$,
$\translIR(\coop{A} \Next\phi) = \langle A \rangle\translIR(\phi)$,
$\translIR(\coop{A} \Always\phi) = \nu X(\translIR(\phi) \land \langle A \rangle X)$,
$\translIR(\coop{A} \psi\Until\phi) =
\mu X(\translIR(\phi) \lor ( \translIR(\psi) \land \langle A \rangle X))$,
where $p\in\Props$, $\phi,\psi\in\ATL$, and $A\subseteq\Agt$.

It is known~\cite{AlurHK02} that $\model,q\satisf[\IR]\phi$ iff
$\model,q\modelsmu\translIR(\phi)$,
for each $\phi\in\ATL$ and $q\in\States$. Indeed, fixed-point computations
are the usual way of verifying $\ATL$.
As shown in~\cite{BullingJ11}, this approach does not extend to
\ATLir and \afAMCi.
The fact that these logics are of incomparable expressivity
means that model checking of \afAMCi cannot be used, in general, for
model checking of \ATLir.
%
Let us illustrate this on the example of reachability.

\subsection{Reachability in ATL\textsubscript{\lowercase{ir}} versus
\lowercase{af}-AMC\textsubscript{\lowercase{i}}}

%\paragraph{First Problems With Reachability}

It is not obvious how to define the reachability for \afAMCi.
A straightforward imitation of the fixed-point definition % of the modality $\Sometm$
from $\ATL$ immediately proves problematic.
Namely, if we introduce a new derived modality $\futmodwhat$ in such a way that
$\coop{A}\futmodwhat\phi\equiv
\mu X(\phi \lor \diam{A} X)$,
then it is easy to observe that
$\model,q\modelsirmu\phi$ implies
$\model,q\modelsirmu\coop{A}\futmodwhat\phi$.
This, however, is inconsistent with \ATLir, where
$\model,q\satisf[\ir]\phi\implies \model,q\satisf[\ir]\coop{A}\Sometm\phi$
does not hold.
On the other hand, we have
$\model,q\satisf[\ir]\everyknowmod_A\phi\implies \model,q\satisf[\ir]\coop{A}\Sometm\phi$,
i.e., if the coalition $A$ knows $\phi$, then $\phi$ is bound to happen, as it is actually occurring.
This suggests the following definition:
\begin{equation*}
\diam{A} \futmoddamn\phi \equiv \mu X(\everyknowmod_A\phi \lor \diam{A} X),
\end{equation*}
for all $A\subseteq\Agt$, $\phi\in\afAMCi$.
However, as we show in the following proposition, this still does not capture the
concept of $ir$--reachability.

%\paragraph{Further Problems With Reachability}

%% In the following theorem we characterise the correspondence (or rather, the lack of it)
%% between the reachability in \ATLir and \afAMCi.

\begin{proposition}\label{thmreach}
Let $A\subseteq\Agt$, $q\in\States$, ${p}\in\Props$, and $\xval\in\xvarsvals$. The following conditions hold:
\begin{enumerate}
\item $\model,q\modelsirmu\coop{\emptyset}\futmoddamn{p}$ iff $\model,q\satisf[\ir]\coop{\emptyset}\Sometm{p}$, \label{thmreachcase1}
\item if $|A| = 1$, then
$\model,q\modelsirmu\coop{A}\futmoddamn{p}$ implies $\model,q\satisf[\ir]\coop{A}\Sometm{p}$,
but the reverse implication is not true,
\label{thmreachcase2}
\item if $|A| > 1$, then
$\model,q\modelsirmu\coop{A}\futmoddamn{p}$ does not imply $\model,q\satisf[\ir]\coop{A}\Sometm{p}$,
and the reverse implication is not true too. \label{thmreachcase3}
\end{enumerate}
\end{proposition}
\begin{proof}
The first case follows from the fact that for the empty coalition
of agents the $ir$--reachability is equivalent to the $IR$--reachability,
which in turn has a fixed-point characterisation in $\AMC$~\cite{AlurHK02}.
For the empty coalition, this characterisation carries over to \afAMCi.

Let us move to the second case.
We define the sequence $\{F_j\}_{j\in\Nat}$ of formulae of \afAMCi such that
$F_0 = \knowmod_a{p}$ and $F_{j+1} = F_0 \lor \diam{A} F_j$, for all $j\ge 0$.
From Kleene fixed-point theorem we have
$\denotation{\coop{a}\Sometm{p}}^\model_{\mu{}ir} = \bigcup_{j=0}^\infty \denotation{F_j}^\model_{\mu{}ir}$,
where $\{\denotation{F_j}^\model_{\mu{}ir}\}_{j\in\Nat}$ is a non-decreasing monotone
sequence of subsets of $\States$.
%
%% For our convenience let us introduce the following notation:
%% for $Q\subseteq\States$ and an equivalence relation $\sim$ on $\States$
%% we denote $\cls(Q,\sim) = \bigcup_{q\in Q} [q]_\sim$.
%
Now, we prove that for each $j\in\Nat$ there exists a partial strategy $s_a^j$ such that
$dom(s_a^{j}) = \denotation{F_{j}}^\model_{\mu{}ir}$, $\forall q\in dom(s_a^j) \;\forall\lambda\in \outir_{\model}(q, s_a^j)\; \exists{k\le j} \;\lambda_k\modelsirmu{p}$,
              and $s_a^j\subseteq s_a^{j+1}$.
%
The proof is by induction on $j$. We constructively build $s_a^{j+1}$ from $s_a^j$ for each $j\in\Nat$.
The base case is trivial.
For the inductive step, firstly observe that for each $j\in\Nat$ if $q\in\denotation{F_j}^\model_{\mu{}ir}$, then
$[q]_{\sim_a}\subseteq\denotation{F_j}^\model_{\mu{}ir}$.
Due to the fact that $\sim_a$ is an equivalence relation,
for each $q\in F_{j+1}$ either $[q]_{\sim_a}\subseteq F_j$ or
$[q]_{\sim_a}\subseteq F_{j+1}\setminus F_j$.
%
In the first case we put $s_a^{j+1}(q) = s_a^j(q)$.
In the second case, we know that there exists a strategy $s_a^{q}$ such that
$\forall\lambda\in \outir_{\model}(q, s_a^{q})\; \lambda_1\in\denotation{F_j}^\model_{\mu{}ir}$.
Moreover, due to the fact that $\sim_a$ is an equivalence relation, the set of such strategies
is shared by the whole class $[q]_{\sim_a}$. We therefore put $s_a^{j+1}(q') = s_a^{q}(q')$ for all
$q'\in[q]_{\sim_a}$.
%
Finally, we can define the partial strategy $s_a = \bigcup_{j\in\Nat}s_a^j$.
For each $q\in\States$ such that
$\model,q\modelsirmu\coop{A}\futmoddamn{p}$,
either $\model,q\modelsirmu{p}$, or ${p}$ will be reached
along each path consistent with any extension of $s_a$ to a full
strategy.
%
The fact that the reverse implication is not true is shown in~\cite{BullingJ11} (Proposition 4).

\input{antipic}
We now move to the last case and consider the \ICGS\ $\model_1$ presented in
Fig.~\ref{rysanty}. We assume that $\prot_1(s) = \{a,b\}$ and
$\prot_2(s) = \{x,y\}$, for $s\in\{t,v,r,u\}$. In the remaining states the protocols
allow only one transition.
For clarity, we omit from the figure the transitions leaving the
states $t,v,r$, and $u$, leading to $\sink$.
By hand-calculations one can observe that
$\model,q\modelsirmu\coop{1,2}\futmoddamn p$
and
$\model,q\not\satisf[\ir]\coop{1,2}\Sometm p$.
This example can be easily extended with a larger number of
(idle) agents.
This concludes the proof of the case and the proposition.
\end{proof}

\subsection{Altering the Next-Step Operator}

\input{reaspic}

From the practical point of view, the results obtained so far are rather discouraging.
A logic based on fixed-points such as \afAMCi may enable more efficient procedures
of model checking than \ATLir, especially if the computations can be performed locally,
i.e., without enumerating over the entire statespace. 
However, as shown in Proposition~\ref{thmreach},
the verification of the formulae of \ATLir by their natural translation to
\afAMCi does not work in general.

%
In what follows, we propose a new version of the next-step operator, denoted by $\diamPImp{\cdot}$.
As we show, this construct retains the basic properties of the next-step operator of \ATLir
%The main benefit of this new operator consists however in the fact that
and the fixed-point reachability
defined using $\diamPImp{\cdot}$ %in the usual way
implies $ir$--reachability.

Let $A\subseteq\Agt$. Following~\cite{FaginHMV95} we define the relation of the \emph{common knowledge} as
$\sim_C^A = (\sim_E^A)^\star$, where ${}^\star$ is the operator of transitive closure.
We define the modality of \emph{common knowledge} $\commonknowmod_A$ in such a way
that $\model,q\models\commonknowmod_A\phi$
iff $\model,q'\models\phi$ for all $q'\sim_C^A q$.
%
For our convenience, and with a slight notational abuse ($\sim_E^A$ is not an equivalence relation),
we denote $[q]_{\sim_E^A} = \{q'\in\States\mid q'\sim_E^A q\}$.


\paragraph{Persistent Next-Step Operator}
Before we present the goal construct, we introduce
an intermediate next-step operator
$\diamPers{\cdot}$ whose aim is to alleviate the following limitation of \afAMCi.
Consider the single-agent \ICGS\ presented in Fig.~\ref{reaspic}.
Observe that the sole possible strategy, in which 
agent $1$ selects action $a$, enforces eventually reaching $p$, i.e.,
$\model_2,q\satisf[\ir]\coop{1}\Sometm p$.
On the other hand, $\model_2,q\not\modelsirmu\coop{1}\futmoddamn p$.
The reason for the latter is that the next-step operator \ATLir
requires reaching $p$ in the succeeding state from \emph{all} the states indistinguishable
from $q$, whereas $p$ is reached from $t,q,v$ in zero, one, and two steps, respectively.


Let $s_A\in\strats_A$ be a strategy for $A\subseteq\Agt$ and
$Q\subseteq\States$. From
$\model = \langle\Agt, \States, \Props, \V, \Actions, \prot, \outf, \{\sim_a\mid a\in\Agt\} \rangle$
we build the restricted model
$\model_{s_A}^Q = \langle\Agt, \States, \Props', \V', \Actions, \prot', \outf', \{\sim_a\mid a\in\Agt\} \rangle$
as follows.
Firstly, in each state $q\in\States$ and agent $a\in A$ we limit the set of actions allowed
to $a$ to the one selected by $s_a$, i.e., $\prot_a(q)' = \{s_a(q)\}$.
Secondly, we introduce a new, fresh proposition $\qprop$ with labeling $\V'(\qprop) = Q$.
All the remaining components of $\model_{s_A}^Q$ are inherited from $\model$.

Let $q\in\States$, $\xval\in\xvarsvals$, and $\phi\in\afAMCi$.
We define the auxilliary operator $\afmod$ by giving its denotation function as follows:
\begin{equation*}\label{afmoddef}
\denotation{\afmod_Q^{s_A}\phi}^\model_{\mu{}ir,\xval}
= \{q\in\States\mid \model_{s_A}^Q,q\models \qprop\land \coop{\emptyset}\qprop\Until \phi\}.
\end{equation*}
Intuitively, $\model,q\modelsirmu\afmod_Q^{s_A}\phi$ iff $q\in Q$ and all the paths starting
in $q$ eventually reach $\phi$ without leaving $Q$ (except for the last step, possibly).

Now we are ready to define the new operator, called the \emph{persistent next-step operator} $\diamPers{\cdot}$.
Its denotation function is as follows:
\begin{equation*}\label{pnextstepdef}
\denotation{\diamPers{A}\phi}^\model_{\mu{}ir,\xval}
\!=\! \{q\in\States\mid \exists{s_A\in\strats_A} \;\denotation{\afmod_{[q]_{\sim_E^A}}^{s_A}\phi}^\model_{\mu{}ir,\xval} \!=\! [q]_{\sim_E^A}\},
\end{equation*}
where $A\subseteq\Agt$.
Observe that
$\model,q\modelsirmu \diamPers{A}\phi$ iff there exists a strategy $s_A\in\strats_A$ such that
every outcome $\lambda\in\outir_{\model}(q, s_A)$ eventually reaches $\phi$ without leaving $[q]_{\sim_E^A}$.
We therefore have the following proposition.

\begin{proposition}
Let $A\subseteq\Agt$, %$\xval\in\xvarsvals$,
$q\in\States$, and ${p}\in\Props$.
If $\model,q\modelsirmu \diamPers{A}{p}$,
then $\model,q\satisf[\ir]\coop{A}\Sometm{p}$.
\end{proposition}

However, the operator of the persistent next-step is only an
intermediate step of our construction. Let us define
the new \emph{persistent reachability} operator $\SometmPers$
in the usual way, by putting
$\diam{A}\SometmPers\phi \equiv \mu X(\everyknowmod_A\phi \lor \diamPers{A} X)$.
One can observe that $\model,q\modelsirmu\diam{A}\phi$
implies $\model,q\modelsirmu \diamPers{A}\phi$,
hence we have the following proposition.

\begin{proposition}
Let $A\subseteq\Agt$, %$\xval\in\xvarsvals$,
$q\in\States$, and ${p}\in\Props$.
$\model,q\modelsirmu \coop{A}\SometmPers{p}$
does not imply $\model,q\satisf[\ir]\coop{A}\Sometm{p}$.
\end{proposition}

Indeed, in the \ICGS\ presented in Fig.~\ref{rysanty}
we have $\model,q\modelsirmu \coop{A}\SometmPers p$
and $\model,q\not\satisf[\ir] \coop{A}\Sometm p$.
Recall that the method of unification of strategies for the case of single agent,
presented in the proof of Proposition~\ref{thmreach}, was based on the fact that the relation
of everybody knows $\sim_A$ is an equivalence relation if $|A| = 1$.
We thus alter the definition of the persistent next-step operator
%given in Eq.~\ref{pnextstepdef}
by putting the relation of common knowledge in place of everybody knows
to obtain the next type of the next-step operator.

\paragraph{Persistent Imperfect Next-Step Operator}

%Let $\phi\in\afAMCi$, $A\subseteq\Agt$, and $\xval\in\xvarsvals$.
We define the \emph{persistent imperfect next-step operator} $\diamPImp{\cdot}$ by
giving its denotation function:
\begin{equation*}\label{punextstepdef}
\denotation{\diamPImp{A}\phi}^\model_{\mu{}ir,\xval}
\!=\! \{q\!\in\!\States\mid\exists{s_A\in\strats_A} \;\denotation{\afmod_{[q]_{\sim_C^A}}^{s_A}\phi}^\model_{\mu{}ir,\xval} = [q]_{\sim_C^A}\},
\end{equation*}
where $\phi\in\afAMCi$, $A\subseteq\Agt$, and $\xval\in\xvarsvals$.
%
Intuitively, $\model,q\modelsirmu \diamPImp{A}\phi$
if the coalition $A$ has the common knowledge that $\phi$ is happening either now or in the next step.
As previously, let us define a new, derived modality $\SometmPImp$ as follows:
\begin{equation*}
\diam{A} \SometmPImp\phi \equiv \mu X(\everyknowmod_A\phi \lor \diamPImp{A} X),
\end{equation*}
for all $A\subseteq\Agt$, $\phi\in\afAMCi$.
As shown in the following theorem, this type of reachability implies $ir$--reachability.

\begin{theorem}\label{reachthm}
Let $A\subseteq\Agt$, $q\in\States$, $\phi\in\Props$, and $\xval\in\xvarsvals$.
If $\model,q\modelsirmu\coop{A}\SometmPImp\phi$, then $\model,q\satisf[\ir]\coop{A}\Sometm\phi$.
%The reverse implication does not hold.
\end{theorem}

\begin{proof}
The proof is similar to the proof of Proposition~\ref{thmreach}.
As previously, let us define the sequence $\{F_j\}_{j\in\Nat}$
of formulae of \afAMCi such that $F_0 = \everyknowmod_A{p}$
and $F_{j+1} = F_0 \lor \diamPImp{A} F_j$, for all $j\ge 0$.
In our proof we use the derived sequence $\{H_j\}_{j\in\Nat}$
of formulae of \afAMCi such that
$H_j = \diamPImp{A} F_j$ for all $j\in\Nat$.
%
From Kleene fixed-point theorem we have
$\denotation{\coop{A}\SometmPImp{p}}^\model_{\mu{}ir}
= \denotation{F_0}^\model_{\mu{}ir} \cup \bigcup_{j=0}^\infty \denotation{H_j}^\model_{\mu{}ir}$.
%
Observe that due to the fact that $\sim_C^A$ is an equivalence relation, for each $q\in\States$
and $j\in\Nat$,
if $[q]_{\sim_C^A}\cap \denotation{H_{j}}^\model_{\mu{}ir} \ne \emptyset$, then
$[q]_{\sim_C^A}\subseteq \denotation{H_{j}}^\model_{\mu{}ir}$.

We prove that for each $j\in\Nat$ there exists a partial strategy $s_A^j$ such that
$dom(s_A^{j}) = \denotation{H_{j}}^\model_{\mu{}ir}$,
$\forall q\in dom(s_A^j) \;\forall\lambda\in \outir_{\model}(q, s_A^j)\; \exists k\in\Nat\;\lambda_k\modelsirmu\everyknowmod_A{p}$,
and $s_A^j\subseteq s_A^{j+1}$.
%
The proof is by induction on $j$. In the base case of $H_0 = \diamPImp{A} \everyknowmod_A{p}$
observe that if $q\in \denotation{H_0}^\model_{\mu{}ir}$ then there exists
a partial strategy $s_A^{0,q}$ with $dom(s_A^{0,q}) = [q]_{\sim_C^A}$ such that every
$\lambda\in \outir_{\model}(q, s_A^{0,q})$ stays in $[q]_{\sim_C^A}$ until it reaches a state where $\everyknowmod_A{p}$ holds.
As $\sim_C^A$ is an equivalence relation, we can now
define $s_A^{0} = \bigcup_{[q]_{\sim_C^A} \in \States/\sim_C^A} s_A^{0,q}$, where any choice of the representative
from a given abstraction class is correct.
%
For the inductive step, we divide the construction of $s_A^{j+1}$ in two cases.
Firstly, if $q\in\denotation{H_j}^\model_{\mu{}ir}$, then we put $s_A^{j+1}(q) = s_A^{j}(q)$.
Secondly, let $q\in\denotation{H_{j+1}}^\model_{\mu{}ir}\setminus\denotation{H_j}^\model_{\mu{}ir}$.
In this case there exists a partial strategy $s_A^{j+1,q}$ with
$dom(s_A^{j+1,q}) = [q]_{\sim_C^A}$ such that each outcome $\lambda\in \outir_{\model}(q, s_A^{j+1,q})$
stays in $[q]_{\sim_C^A}$ until it reaches a state $q'$ in which either $\everyknowmod_A{p}$ holds
or $q'\in \denotation{H_j}^\model_{\mu{}ir}$.
In the latter case from the inductive assumption we know that following $s_A^{j+1}$ (i.e., $s_A^{j}$, by
the previous case) always leads to reaching $\everyknowmod_A{p}$
without leaving $\denotation{H_j}^\model_{\mu{}ir}$.
%
We therefore put
$s_A^{j+1} = \bigcup_{[q]_{\sim_C^A} \in \States/\sim_C^A} s_A^{j+1,q}$, where, again, any choice of the representative
from an abstraction class is correct.

Finally, we can build a partial strategy $s_A = \bigcup_{j\in\Nat} s_A^j$.
Any extension $s_A'$ of this strategy is such that
for each $q\in\States$, if
$\model,q\modelsirmu\coop{A}\SometmPImp{p}$
then a state in which $\everyknowmod_A{p}$ holds is eventually reached
along each outcome $\lambda\in \outir_{\model}(q, s_A')$.
This concludes the proof.
\end{proof}

\subsection{Approximating ATL\textsubscript{\lowercase{ir}}}

We now extend the approach presented above to approximate the full language of
\ATLir. To this end we define a new logic, called
Approximative Alternating-Time Temporal Logic with Imperfect Information and Recall
(\ATL[ira], for short). Similarly to \ATLir, \ATL[ira] shares the syntax with
$\ATL$ (cf. Definition~\ref{atlsyntax}) and
its semantics is based on the persistent imperfect next-step operator.
We denote the satisfaction relation in \ATL[ira] by $\satisf[ira]$.

\begin{definition}[{\ATL[ira]} Semantics]
The semantics of \ATL[ira] is defined as follows (we omit the boolean
operations and the next-step operator, whose semantics is inherited from \ATLir):
\begin{itemize}
%% \item $\model,q\satisf[ira]\coop{A} \Next\phi$ iff
%% $\model,q\modelsirmu\diam{A}\phi$,
\item $\model,q\satisf[ira]\coop{A} \Always\phi$ iff
$\model,q\modelsirmu\nu X(\commonknowmod_A\phi \land \diamPImp{A} X)$,
\item $\model,q\satisf[ira]\coop{A} \psi\Until\phi$ iff
$\model,q\modelsirmu\mu X\big(\everyknowmod_A\phi \lor(\commonknowmod_A\psi \land \diamPImp{A} X)\big)$,
\end{itemize}
where $q\in\States$, $p\in\Props$, $\phi,\psi\in\ATLir$, and $A\subseteq\Agt$.
\end{definition}

Observe that $\coop{A}\SometmPImp\phi \equiv \coop{A} \true\Until\phi$.
We say that a formula is in \emph{positive normal form} if the negation is applied only to propositions.
As shown in the following theorem, \ATL[ira] underapproximates \ATLir, when limited
to the formulae in positive normal form.

\begin{theorem}
Let $A\subseteq\Agt$, $q\in\States$, and $\phi\in\ATL$ be in positive normal form.
If $\model,q\satisf[ira]\phi$, then $\model,q\satisf[\ir]\phi$.
\end{theorem}

\begin{proof}
The proof is by induction on the structure of $\phi$. We omit the easy cases of boolean operations
and the next-step operator. We also omit the proof of case of $\coop{A} \psi\Until\phi$,
as it is very similar to the proof of Theorem~\ref{reachthm}.

We therefore focus on $\coop{A} \Always\phi$.
%
Let us define the sequence $\{G_j\}_{j\in\Nat}$ of formulae such that
$G_0 = \commonknowmod_A\phi$ and $G_{j+1} = G_0 \land \diamPImp{A} G_j$,
for all $j\ge 0$.
From Kleene fixed-point theorem we have
$\denotation{\coop{A}\Always\phi}^\model_{ira} = \bigcap_{j=0}^\infty \denotation{G_j}^\model_{ira}$.
%
It suffices to prove that for each $j\in\Nat$ there exists a strategy $s_A^j$ such that
$\forall q\in \denotation{G_j}^\model_{ira} \;\forall\lambda\in \outir_{\model}(q, s_A^j)\; \forall{0\le k\le j} \;\lambda_k\satisf[ira]\phi$.
This proof is by induction on $j$, with the trivial base case.
%
Assume that the inductive assumption holds for some $j\in\Nat$.
%
From the definition of the persistent imperfect next-step operator
we can define for each equivalence class $[q]_{\sim_C^A}\in \denotation{G_{j+1}}^\model_{ira}/\sim_C^A$
a partial strategy $s_{A}^{[q]_{\sim_C^A}, j+1}$ such that
$\forall q\in [q]_{\sim_C^A}\;\forall\lambda\in \outir_{\model}(q, [q]_{\sim_C^A}) \;\lambda_1\in\denotation{G_j}^\model_{ira}$.
We now build
$s_{A}^{j+1} = \bigcup_{[q]_{\sim_C^A}\in \denotation{G_{j+1}}^\model_{ira}/\sim_C^A} s_{A}^{[q]_{\sim_C^A}, j+1}
\cup
{s_{A}^j}_{|\denotation{\commonknowmod_A\phi}^\model_{ira}\setminus\denotation{G_j}^\model_{ira}}
$.
Intuitively, $s_{A}^j$ enforces that a path leaving each $q\in\denotation{G_{j+1}}^\model_{ira}$
stays within $\denotation{\commonknowmod_A\phi}^\model_{ira}$
for either infinite number of steps (it then visits $\denotation{G_j}^\model_{ira}$
infinitely often) or at least $j$ number of steps in
$\denotation{G_{j}}^\model_{ira}\setminus\denotation{G_{j+1}}^\model_{ira}$.
Note that the correctness of the above definition stems from the fact that $\sim_C^A$ is
an equivalence relation.
\end{proof}

In fact, a closer inspection of the above proof shows that a stronger result can be obtained.
Namely, if we define a new logic by extending \ATLir with the operator of
common knowledge (recall~\cite{BullingJ11} that the everybody knows operator
is a derived modality in \ATLir), then:

\begin{itemize}
\item $\model,q\satisf[ira]\coop{A} \Always\phi$
implies
$\model,q\satisf[\ir]\coop{A} \Always\commonknowmod_A\phi$,
\item $\model,q\satisf[ira]\coop{A} \psi\Until\phi$
implies
$\model,q\satisf[\ir]\coop{A} \everyknowmod_A\psi\Until\commonknowmod_A\phi$.
\end{itemize}


==> reaspic.tex <==
\tikzstyle{every state} = []
\def\stpd{5.0}
\node[state, initial above] (s0) at (0.0, 0.0) {$q$};
\node[state] (s1) at (3.0, 0.0) {$v$};
\node[state, label=-90:{$p$}] (s2) at (0.0, -2.0) {};
\node[state, label=-90:{$p$}] (s3) at (-3.0, 0.0) {$t$};

 \path [-,style=dashed,shorten >=1pt, auto, node distance=7cm, semithick]
(s0) edge node {1} (s1)
(s0) edge node {1} (s3)

;

\path [->,style=solid,shorten >=1pt, auto, node distance=7cm, semithick]
(s0) edge node {$a$} (s2)
(s1) edge [bend right] node [above] {$a$} (s0)

(s2) edge [loop left] (s2)
%(s3) edge [loop left] (s3)
;


==> response___notes.tex <==
We thank the reviewers for all their remarks.

Addressing specific comments:

(Q1) Yes, tr_1 should provide a correct lower bound for <<a>>_ir F\phi in the objective semantics, as long as <A> in the translation is interpreted according to the subjective semantics. Thank you for pointing this out!

(Q2) The existing benchmarks (TianJi and Castles) were not used in the experimental evaluation not because there is anything wrong with them, but because they do not satisfy some applicability conditions for our approach. In other words, our approach is bound to be useless for those benchmarks. If a model does not satisfy condition (2) of Proposition 10, then the fixpoint translations tr_2 and tr_3 will always return *false*. As a lower bound, this brings no useful information about the real value of \phi.

- Abstraction classes are indeed equivalence classes. We will unify the terminology.

- Translation of properties on p.7: right, the English explanation does not express what we intended. We will correct that.

(NOTES:

- p.3: "use model M3 from Fig 3B" -- p must not hold in q2 for the argument to hold!

)


==> results-bridge-absentminded.tex <==
\hspace{-0.7cm}\resizebox{1.15\columnwidth}{!}{%
\begin{tabular}{|c|HHHc|Hc|Hc|Hc|Hc|Hc|c|c|}
\hline
\multirow{2}{*}{$(n,k)$} & \multirow{2}{*}{btime}    & \multirow{2}{*}{\#bsat} & \multirow{2}{*}{rtime}    & \multirow{2}{*}{\#states}  & \multirow{2}{*}{eptime}   & \multirow{2}{*}{tgen}
  & \multicolumn{4}{c|}{Lower approx.\extended{ (\AEMC)}}           & \multicolumn{4}{c|}{Upper approx.\extended{ (\ATLIr)}}      &  \multirow{2}{*}{Match}   &    Exact   \\
\cline{8-15}
\cline{17-17}
  &  &  &  &  &  &  & \#iter & tverif     & \#sat   & \%true & \#iter & tverif   & \#sat   & \%true &  &  tg+tv \\
\hline
\hline
$(1,1)$           & {5.24e-05} & {2}      & {1.16e-03} & {19}     & {9.89e-06} & 0.001 & 2      & 0.0003 & 19    & 100\%  & 4      & 0.0003 & 19    & 100\%   & {100\%}    & {14.59\,h}$^\star$ \\ \hline
$(2,2)$           & {1.59e-04} & {6}      & {6.78e-02} & {774}    & {1.75e-04} & 0.07 & 2      & 0.01 & 383   & 40\%   & 6      & 0.02 & 410   & 50.00\% & {90\%}     & \tmout        \\ \hline
$(3,3)$           & {7.86e-04} & {20}     & {6.70}     & {51865}  & {9.85e-03} & 6.71     & 5      & 29.31    & 20757 & 65\%   & 11     & 2.45     & 23818 & 85\%    & {80\%}     & \tmout        \\ \hline
\end{tabular}%
}


==> results-bridge-old.tex <==
\hspace{-0.6cm}\resizebox{1.15\columnwidth}{!}{%
\begin{tabular}{|@{\,}c@{\,}|HHHc|Hc|Hc|Hc|Hc|Hc|c|c|}
\hline
\multirow{2}{*}{$(n,k)$} & \multirow{2}{*}{btime}    & \multirow{2}{*}{\#bsat} & \multirow{2}{*}{rtime}    & \multirow{2}{*}{\#states}  & \multirow{2}{*}{eptime}   & \multirow{2}{*}{tgen}
  & \multicolumn{4}{c|}{Lower approx.\extended{ (\AEMC)}}           & \multicolumn{4}{c|}{Upper approx.\extended{ (\ATLIr)}}      &  \multirow{2}{*}{Match}   &    Exact   \\
\cline{8-15}
\cline{17-17}
  &  &  &  &  &  &  & \#iter & tverif     & \#sat   & \%true & \#iter & tverif   & \#sat   & \%true &  &  tg+tv \\
\hline
\hline
$(1,1)$           & {3.15e-05} & {2}      & {3.29e-04} & {11}      & {1.81e-04} & 0.0005 & 5      & 0.0001 & 11      & 100\%  & 5      & 7e-05 & 11      & 100\%  & {100\%}    & {0.19}   \\ \hline
$(2,2)$           & {9.05e-05} & {6}      & {1.15e-02} & {310}     & {5.37e-03} & 0.017 & 9      & 0.002 & 184     & 60\%   & 9      & 0.001 & 184     & 60\%   & {100\%}    & {2.42\,h}$^\star$%$^\diamond$
\\ \hline
$(3,3)$           & {3.38e-04} & {20}     & {0.65}     & {12626}   & {0.27}     & 0.92     & 13     & 0.16     & 5672    & 70\%   & 14     & 0.05 & 5929    & 70\%   & {100\%}    & \tmout       \\ \hline
$(4,4)$           & {1.74e-02} & {70}     & {31.22}    & {534722}  & {10.43}    & 41.66    & 19     & 172.07   & 225091  & 60\%   & 19     & 2.61     & 233520  & 60\%   & {100\%}    & \tmout       \\ \hline
$\;(5,5)^\star$           & {5.07e-02} & {252}    & {2449.45}  & {2443467} & {192.36}   & 2641.86  & 15     & 76 h     & 2443467 & 100\%   & 15     & 1929     & 2443467 & 100\%   & {100\%}    & \tmout       \\ \hline
\end{tabular}%
} 
